A Comprehensive Study of Ly$\alpha$ Emission in the High-redshift Galaxy Population

We present an exhaustive census of Lyman alpha (Ly$\alpha$) emission in the general galaxy population at $3<z<4.6$. We use the Michigan/Magellan Fiber System (M2FS) spectrograph to study a stellar mass (M$_*$) selected sample of 625 galaxies homogeneously distributed in the range $7.6<\log{\mbox{M$_*$/M$_{\odot}$}}<10.6$. Our sample is selected from the 3D-HST/CANDELS survey, which provides the complementary data to estimate Ly$\alpha$ equivalent widths ($W_{Ly\alpha}$) and escape fractions ($f_{esc}$) for our galaxies. We find both quantities to anti-correlate with M$_*$, star-formation rate (SFR), UV luminosity, and UV slope ($\beta$). We then model the $W_{Ly\alpha}$ distribution as a function of M$_{UV}$ and $\beta$ using a Bayesian approach. Based on our model and matching the properties of typical Lyman break galaxy (LBG) selections, we conclude that the $W_{Ly\alpha}$ distribution in such samples is heavily dependent on the limiting M$_{UV}$ of the survey. Regarding narrowband surveys, we find their $W_{Ly\alpha}$ selections to bias samples toward low M$_*$, while their line-flux limitations preferentially leave out low-SFR galaxies. We can also use our model to predict the fraction of Ly$\alpha$-emitting LBGs at $4\leqslant z\leqslant 7$. We show that reported drops in the Ly$\alpha$ fraction at $z\geqslant6$, usually attributed to the rapidly increasing neutral gas fraction of the universe, can also be explained by survey M$_{UV}$ incompleteness. This result does not dismiss reionization occurring at $z\sim7$, but highlights that current data is not inconsistent with this process taking place at $z>7$.

==> bibliografia.tex <==
\begin{thebibliography}{100}
\bibitem[Adams et al.(2011)]{2011ApJS..192....5A} Adams, J.~J., Blanc, G.~A., Hill, G.~J., et al.\ 2011, \apjs, 192, 5 
\bibitem[Atek et al.(2014)]{2014AA...561A..89A} Atek, H., Kunth, D., Schaerer, D., et al.\ 2014, \aap, 561, A89
\bibitem[Balestra et al.(2010)]{2010AA...512A..12B} Balestra, I., Mainieri, V., Popesso, P., et al.\ 2010, \aap, 512, A12
\bibitem[Bennett et al.(2013)]{2013ApJS..208...20B} Bennett, C.~L., Larson, D., Weiland, J.~L., et al.\ 2013, \apjs, 208, 20
\bibitem[Blanc et al.(2011)]{2011ApJ...736...31B} Blanc, G.~A., Adams, J.~J., Gebhardt, K., et al.\ 2011, \apj, 736, 31
\bibitem[Bond et al.(2012)]{2012ApJ...753...95B} Bond, N.~A., Gawiser, E., Guaita, L., et al.\ 2012, \apj, 753, 95 
\bibitem[Boquien et al.(2014)]{2014AA...571A..72B} Boquien, M., Buat, V., \& Perret, V.\ 2014, \aap, 571, A72 	
\bibitem[Bouwens et al.(2007)]{2007ApJ...670..928B} Bouwens, R.~J., Illingworth, G.~D., Franx, M., \& Ford, H.\ 2007, \apj, 670, 928
\bibitem[Bouwens et al.(2012)]{2012ApJ...754...83B} Bouwens, R.~J., Illingworth, G.~D., Oesch, P.~A., et al.\ 2012, \apj, 754, 83
\bibitem[Bouwens et al.(2014)]{2014ApJ...793..115B} Bouwens, R.~J., Illingworth, G.~D., Oesch, P.~A., et al.\ 2014, \apj, 793, 115
\bibitem[Brammer et al.(2008)]{2008ApJ...686.1503B} Brammer, G.~B., van Dokkum, P.~G., \& Coppi, P.\ 2008, \apj, 686, 1503-1513
\bibitem[Calzetti et al.(1994)]{1994ApJ...429..582C} Calzetti, D., Kinney, A.~L., \& Storchi-Bergmann, T.\ 1994, \apj, 429, 582
\bibitem[Calzetti et al.(2000)]{2000ApJ...533..682C} Calzetti, D., Armus, L., Bohlin, R.~C., et al.\ 2000, \apj, 533, 682
\bibitem[Caminha et al.(2015)]{2015arXiv151205655C} Caminha, G.~B., Karman, W., Rosati, P., et al.\ 2015, arXiv:1512.05655
\bibitem[Cassata et al.(2011)]{2011AA...525A.143C} Cassata, P., Le F{\`e}vre, O., Garilli, B., et al.\ 2011, \aap, 525, A143
\bibitem[Cassata et al.(2015)]{2015AA...573A..24C} Cassata, P., Tasca, L.~A.~M., Le F{\`e}vre, O., et al.\ 2015, \aap, 573, A24
\bibitem[Chabrier(2003)]{2003PASP..115..763C} Chabrier, G.\ 2003, \pasp, 115, 763 
\bibitem[Charlot \& Fall(1993)]{1993ApJ...415..580C} Charlot, S., \& Fall, S.~M.\ 1993, \apj, 415, 580
\bibitem[Chonis et al.(2013)]{2013ApJ...775...99C} Chonis, T.~S., Blanc, G.~A., Hill, G.~J., et al.\ 2013, \apj, 775, 99 
\bibitem[Ciardullo et al.(2014)]{2014ApJ...796...64C} Ciardullo, R., Zeimann, G.~R., Gronwall, C., et al.\ 2014, \apj, 796, 64 	
\bibitem[Daddi et al.(2007)]{2007ApJ...670..156D} Daddi, E., Dickinson, M., Morrison, G., et al.\ 2007, \apj, 670, 156 
\bibitem[Dijkstra \& Kramer(2012)]{2012MNRAS.424.1672D} Dijkstra, M., \& Kramer, R.\ 2012, \mnras, 424, 1672
\bibitem[Dressler et al.(2011)]{2011ApJ...740...71D} Dressler, A., Martin, C.~L., Henry, A., Sawicki, M., \& McCarthy, P.\ 2011, \apj, 740, 71 
\bibitem[Dressler et al.(2015)]{2015ApJ...806...19D} Dressler, A., Henry, A., Martin, C.~L., et al.\ 2015, \apj, 806, 19 
\bibitem[Duncan et al.(2014)]{2014MNRAS.444.2960D} Duncan, K., Conselice, C.~J., Mortlock, A., et al.\ 2014, \mnras, 444, 2960 
\bibitem[Duval et al.(2014)]{2014AA...562A..52D} Duval, F., Schaerer, D., {\"O}stlin, G., \& Laursen, P.\ 2014, \aap, 562, A52 
\bibitem[Fan et al.(2006)]{2006AJ....132..117F} Fan, X., Strauss, M.~A., Becker, R.~H., et al.\ 2006, \aj, 132, 117 
\bibitem[Feldmeier et al.(2013)]{2013ApJ...776...75F} Feldmeier, J.~J., Hagen, A., Ciardullo, R., et al.\ 2013, \apj, 776, 75
\bibitem[Finkelstein et al.(2015)]{2015ApJ...813...78F} Finkelstein, K.~D., Finkelstein, S.~L., Tilvi, V., et al.\ 2015, \apj, 813, 78
\bibitem[Finlator et al.(2007)]{2007MNRAS.376.1861F} Finlator, K., Dav{\'e}, R., \& Oppenheimer, B.~D.\ 2007, \mnras, 376, 1861 
\bibitem[Finlator et al.(2009)]{2009MNRAS.400.1049F} Finlator, K., {\"O}zel, F., Dav{\'e}, R., \& Oppenheimer, B.~D.\ 2009, \mnras, 400, 1049
\bibitem[Furusawa et al.(2016)]{2016ApJ...822...46F} Furusawa, H., Kashikawa, N., Kobayashi, M.~A.~R., et al.\ 2016, \apj, 822, 46
\bibitem[Gonz{\'a}lez et al.(2011)]{2011ApJ...735L..34G} Gonz{\'a}lez, V., Labb{\'e}, I., Bouwens, R.~J., et al.\ 2011, \apjl, 735, L34 
\bibitem[Gonz{\'a}lez et al.(2014)]{2014ApJ...781...34G} Gonz{\'a}lez, V., Bouwens, R., Illingworth, G., et al.\ 2014, \apj, 781, 34 	
\bibitem[Grogin et al.(2011)]{2011ApJS..197...35G} Grogin, N.~A., Kocevski, D.~D., Faber, S.~M., et al.\ 2011, \apjs, 197, 35 
\bibitem[Gronke \& Dijkstra(2016)]{2016arXiv160406805G} Gronke, M., \& Dijkstra, M.\ 2016, arXiv:1604.06805 
\bibitem[Gronwall et al.(2007)]{2007ApJ...667...79G} Gronwall, C., Ciardullo, R., Hickey, T., et al.\ 2007, \apj, 667, 79 
\bibitem[Guaita et al.(2010)]{2010ApJ...714..255G} Guaita, L., Gawiser, E., Padilla, N., et al.\ 2010, \apj, 714, 255 
\bibitem[Hagen et al.(2014)]{2014ApJ...786...59H} Hagen, A., Ciardullo, R., Gronwall, C., et al.\ 2014, \apj, 786, 59 
\bibitem[Hayes et al.(2011)]{2011ApJ...730....8H} Hayes, M., Schaerer, D., {\"O}stlin, G., et al.\ 2011, \apj, 730, 8
\bibitem[Hayes et al.(2013)]{2013ApJ...765L..27H} Hayes, M., {\"O}stlin, G., Schaerer, D., et al.\ 2013, \apjl, 765, L27 
\bibitem[Kennicutt(1998)]{1998ARAA..36..189K} Kennicutt, R.~C., Jr.\ 1998, \araa, 36, 189  
\bibitem[Kennicutt \& Evans(2012)]{2012ARAA..50..531K} Kennicutt, R.~C., \& Evans, N.~J.\ 2012, \araa, 50, 531
\bibitem[Kere{\v s} et al.(2005)]{2005MNRAS.363....2K} Kere{\v s}, D., Katz, N., Weinberg, D.~H., \& Dav{\'e}, R.\ 2005, \mnras, 363, 2
\bibitem[Koekemoer et al.(2011)]{2011ApJS..197...36K} Koekemoer, A.~M., Faber, S.~M., Ferguson, H.~C., et al.\ 2011, \apjs, 197, 36
\bibitem[Kriek et al.(2009)]{2009ApJ...700..221K} Kriek, M., van Dokkum, P.~G., Labb{\'e}, I., et al.\ 2009, \apj, 700, 221
\bibitem[Law et al.(2012)]{2012ApJ...759...29L} Law, D.~R., Steidel, C.~C., Shapley, A.~E., et al.\ 2012, \apj, 759, 29
\bibitem[Mallery et al.(2012)]{2012ApJ...760..128M} Mallery, R.~P., Mobasher, B., Capak, P., et al.\ 2012, \apj, 760, 128 
\bibitem[Mateo et al.(2012)]{2012SPIE.8446E..4YM} Mateo, M., Bailey, J.~I., Crane, J., et al.\ 2012, \procspie, 8446, 84464Y
\bibitem[Matthee et al.(2016)]{2016MNRAS.458..449M} Matthee, J., Sobral, D., Oteo, I., et al.\ 2016, \mnras, 458, 449  
\bibitem[Matsuda et al.(2012)]{2012MNRAS.425..878M} Matsuda, Y., Yamada, T., Hayashino, T., et al.\ 2012, \mnras, 425, 878 
\bibitem[McLinden et al.(2011)]{2011ApJ...730..136M} McLinden, E.~M., Finkelstein, S.~L., Rhoads, J.~E., et al.\ 2011, \apj, 730, 136
\bibitem[McLinden et al.(2014)]{2014MNRAS.439..446M} McLinden, E.~M., Rhoads, J.~E., Malhotra, S., et al.\ 2014, \mnras, 439, 446
\bibitem[Meurer et al.(1999)]{1999ApJ...521...64M} Meurer, G.~R., Heckman, T.~M., \& Calzetti, D.\ 1999, \apj, 521, 64 
\bibitem[Momose et al.(2014)]{2014MNRAS.442..110M} Momose, R., Ouchi, M., Nakajima, K., et al.\ 2014, \mnras, 442, 110 
\bibitem[Nilsson et al.(2009)]{2009MNRAS.400..232N} Nilsson, K.~K., M{\"o}ller-Nilsson, O., M{\o}ller, P., Fynbo, J.~P.~U., \& Shapley, A.~E.\ 2009, \mnras, 400, 232
\bibitem[Noeske et al.(2007)]{2007ApJ...660L..43N} Noeske, K.~G., Weiner, B.~J., Faber, S.~M., et al.\ 2007, \apjl, 660, L43
\bibitem[Oke \& Gunn(1983)]{1983ApJ...266..713O} Oke, J.~B., \& Gunn, J.~E.\ 1983, \apj, 266, 713 
\bibitem[Ono et al.(2012)]{2012ApJ...744...83O} Ono, Y., Ouchi, M., Mobasher, B., et al.\ 2012, \apj, 744, 83
\bibitem[Ouchi et al.(2008)]{2008ApJS..176..301O} Ouchi, M., Shimasaku, K., Akiyama, M., et al.\ 2008, \apjs, 176, 301-330  
\bibitem[Oyarz{\'u}n et al.(2016)]{2016ApJ...821L..14O} Oyarz{\'u}n, G.~A., Blanc, G.~A., Gonz{\'a}lez, V., et al.\ 2016, \apjl, 821, L14
\bibitem[Patr{\'{\i}}cio et al.(2016)]{2016MNRAS.456.4191P} Patr{\'{\i}}cio, V., Richard, J., Verhamme, A., et al.\ 2016, \mnras, 456, 4191
\bibitem[Pentericci et al.(2009)]{2009AA...494..553P} Pentericci, L., Grazian, A., Fontana, A., et al.\ 2009, \aap, 494, 553
\bibitem[Pettini et al.(2002)]{2002ApJ...569..742P} Pettini, M., Rix, S.~A., Steidel, C.~C., et al.\ 2002, \apj, 569, 742 
\bibitem[Pickles(1998)]{1998PASP..110..863P} Pickles, A.~J.\ 1998, \pasp, 110, 863  
\bibitem[Planck Collaboration et al.(2015)]{2015arXiv150201589P} Planck Collaboration, Ade, P.~A.~R., Aghanim, N., et al.\ 2015, arXiv:1502.01589
\bibitem[Quadri et al.(2007)]{2007AJ....134.1103Q} Quadri, R., Marchesini, D., van Dokkum, P., et al.\ 2007, \aj, 134, 1103
\bibitem[Reddy et al.(2016)]{2016arXiv160603452R} Reddy, N.~A., Steidel, C.~C., Pettini, M., Bogosavljevic, M., \& Shapley, A.\ 2016, arXiv:1606.03452
\bibitem[Rivera-Thorsen et al.(2015)]{2015ApJ...805...14R} Rivera-Thorsen, T.~E., Hayes, M., {\"O}stlin, G., et al.\ 2015, \apj, 805, 14 
\bibitem[Schaerer(2003)]{2003A&A...397..527S} Schaerer, D.\ 2003, \aap, 397, 527
\bibitem[Schaerer et al.(2011)]{2011AA...536A..72S} Schaerer, D., de Barros, S., \& Stark, D.~P.\ 2011, \aap, 536, A72
\bibitem[Schenker et al.(2012)]{2012ApJ...744..179S} Schenker, M.~A., Stark, D.~P., Ellis, R.~S., et al.\ 2012, \apj, 744, 179
\bibitem[Shapley et al.(2003)]{2003ApJ...588...65S} Shapley, A.~E., Steidel, C.~C., Pettini, M., \& Adelberger, K.~L.\ 2003, \apj, 588, 65 
\bibitem[Shimasaku et al.(2006)]{2006PASJ...58..313S} Shimasaku, K., Kashikawa, N., Doi, M., et al.\ 2006, \pasj, 58, 313
\bibitem[Shimizu et al.(2011)]{2011MNRAS.418.2273S} Shimizu, I., Yoshida, N., \& Okamoto, T.\ 2011, \mnras, 418, 2273
\bibitem[Silva et al.(1998)]{1998ApJ...509..103S} Silva, L., Granato, G.~L., Bressan, A., \& Danese, L.\ 1998, \apj, 509, 103
\bibitem[Skelton et al.(2014)]{2014ApJS..214...24S} Skelton, R.~E., Whitaker, K.~E., Momcheva, I.~G., et al.\ 2014, \apjs, 214, 24
\bibitem[Stanway et al.(2016)]{2016MNRAS.456..485S} Stanway, E.~R., Eldridge, J.~J., \& Becker, G.~D.\ 2016, \mnras, 456, 485 
\bibitem[Stark et al.(2009)]{2009ApJ...697.1493S} Stark, D.~P., Ellis, R.~S., Bunker, A., et al.\ 2009, \apj, 697, 1493
\bibitem[Stark et al.(2010)]{2010MNRAS.408.1628S} Stark, D.~P., Ellis, R.~S., Chiu, K., Ouchi, M., \& Bunker, A.\ 2010, \mnras, 408, 1628 
\bibitem[Stark et al.(2011)]{2011ApJ...728L...2S} Stark, D.~P., Ellis, R.~S., \& Ouchi, M.\ 2011, \apjl, 728, L2
\bibitem[Steidel et al.(1996)]{1996ApJ...462L..17S} Steidel, C.~C., Giavalisco, M., Pettini, M., Dickinson, M., \& Adelberger, K.~L.\ 1996, \apjl, 462, L17 
\bibitem[Tapken et al.(2007)]{2007AA...467...63T} Tapken, C., Appenzeller, I., Noll, S., et al.\ 2007, \aap, 467, 63 
\bibitem[Tilvi et al.(2014)]{2014ApJ...794....5T} Tilvi, V., Papovich, C., Finkelstein, S.~L., et al.\ 2014, \apj, 794, 5
\bibitem[Treu et al.(2012)]{2012ApJ...747...27T} Treu, T., Trenti, M., Stiavelli, M., Auger, M.~W., \& Bradley, L.~D.\ 2012, \apj, 747, 27
\bibitem[Vanzella et al.(2009)]{2009ApJ...695.1163V} Vanzella, E., Giavalisco, M., Dickinson, M., et al.\ 2009, \apj, 695, 1163
\bibitem[Vargas et al.(2014)]{2014ApJ...783...26V} Vargas, C.~J., Bish, H., Acquaviva, V., et al.\ 2014, \apj, 783, 26
\bibitem[Verhamme et al.(2006)]{2006AA...460..397V} Verhamme, A., Schaerer, D., \& Maselli, A.\ 2006, \aap, 460, 397
\bibitem[Verhamme et al.(2008)]{2008AA...491...89V} Verhamme, A., Schaerer, D., Atek, H., \& Tapken, C.\ 2008, \aap, 491, 89
\bibitem[Whitaker et al.(2012)]{2012ApJ...754L..29W} Whitaker, K.~E., van Dokkum, P.~G., Brammer, G., \& Franx, M.\ 2012, \apjl, 754, L29
\bibitem[Wisotzki et al.(2016)]{2016AA...587A..98W} Wisotzki, L., Bacon, R., Blaizot, J., et al.\ 2016, \aap, 587, A98 
\bibitem[Yamada et al.(2005)]{2005PASJ...57..881Y} Yamada, S.~F., Sasaki, S.~S., Sumiya, R., et al.\ 2005, \pasj, 57, 881
\bibitem[Zheng et al.(2014)]{2014MNRAS.439.1101Z} Zheng, Z.-Y., Wang, J.-X., Malhotra, S., et al.\ 2014, \mnras, 439, 1101 
\bibitem[Zitrin et al.(2015)]{2015ApJ...810L..12Z} Zitrin, A., Labb{\'e}, I., Belli, S., et al.\ 2015, \apjl, 810, L12	
\end{thebibliography}
